Recursive Sketches for Modular Deep Learning

We present a mechanism to compute a sketch (succinct summary) of how a complex modular deep network processes its inputs. The sketch summarizes essential information about the inputs and outputs of the network and can be used to quickly identify key components and summary statistics of the inputs. Furthermore, the sketch is recursive and can be unrolled to identify sub-components of these components and so forth, capturing a potentially complicated DAG structure. These sketches erase gracefully; even if we erase a fraction of the sketch at random, the remainder still retains the `high-weight' information present in the original sketch. The sketches can also be organized in a repository to implicitly form a `knowledge graph'; it is possible to quickly retrieve sketches in the repository that are related to a sketch of interest; arranged in this fashion, the sketches can also be used to learn emerging concepts by looking for new clusters in sketch space. Finally, in the scenario where we want to learn a ground truth deep network, we show that augmenting input/output pairs with these sketches can theoretically make it easier to do so.

==> notes.tex <==
\section{Notes}

\begin{enumerate}
    \item Do we need to handle weighted version of the sketch sub-lemma (that Badih am trying to prove).
    \item How are we going to recover tuple rotators $R_1, R_2, \ldots$? Are they square or rectangular?
    \item How do we figure out the (weighted) \# of eyes in a sketch of a scene?
    If we have all the $r_i$'s and if eye at level 3 has effective weight after multiplying the weights, then the types of all the nodes on the path can be identified, and the corresponding matrices can be inverted.
    How to show? Try to reason about head vector and show that it dominates any noise that might arise because it has enough weight.
    \item Given a scene that has 200 chairs and 500 people, we can roughly figure out the number of chairs and the number of people if the chairs and people are "top-level". (Might be faster to do it with $(I+R)/2$ by just computing an inner product whereas in the $R$ case this might require some unraveling operations.). This requires having equal weights on the top-level concepts.
    \item Weighted dictionary version: might need increase the sketching dimension from $k \log{N}$ to $k \log^2{N}$. Assume that weight of relevant part is $1/\sqrt{2}$ and weight of the ``noise'' part is also $1/\sqrt{2}$. Then relevant part would be concentrated on $k\log{N}$ coordinates out of $k \log^2{N}$ whereas the ``noise'' part is spread out over all the $k^2 \log{N}$ coordinates (because the distribution over the coefficients $x$ is independent of the distribution over the $r$ vectors). Here each module gets weight $1/\sqrt{k}$ at least $\epsilon$ fraction of the time and conditioned on this, it doesn't co-occur with any other specific module at least $\epsilon$ fraction of the times. Now figure out the $r_i$ that satisfy this property.
\end{enumerate}

==> properties.tex <==
\section{Recursive Sketches}\label{sec:recursivesketches}

\subsection{Notation}

In the definitions below, $x$ is a (boolean) vector in $\mathbb{R}^d$ and
$R$ is a (boolean) matrix in $\mathbb{R}^{d \times d}$.

The sparsity of $x$, written $\sparsity{x}$, is the number of non-zero
entries of $x$. The sparsity of $R$, written $\sparsity{R}$, is the
maximum number of non-zero entries in any column of $R$.

Simple example:
- sketches are not passed around, the raw output is passed around (think feed-forward network)
- collection of hardwired reversible blocks, each has a vector output (later: could be a set of attributes, each of which is a vector)
- when a top-level block fires, we compute a recursive sketch of its output.

Example:
FACE module results in object $FACE(output, inputs)$
resulting sketch is $s_{FACE}(output, inputs) = R_{FACE}(s(s(output), s(inputs)))$

Tuple sketch vs Set sketch: set sketch is useful when we see a set of objects in a scene for example there may be 5 cats in a scene so we need to sketch the set of 5 cat-sketches. In this case we want to sketch ${S_1,S_2,..S_k}$. This can be done recursively by using a random hyperplane and partitioning the $S_i$'s into two sets and viewing it is as a pair (tuple) and using $S({Set on left half}, {Set on right half})$

Claim: The tuple/set sketch has the following properties:

\begin{itemize}

\item 
1) if the sketch size $>$ sparsity of an Sketching$input / weight^2$ of that input, then w.h.p. the input can be recovered.
\\
\item 
2) if the sketch is done recursively, weight = product of weights
\\
\item 
3) even if we can't recover because the sketch size is too small, we get a sketch of it. For example if we have a vector of positions of many leaves in a tree. The sketch of the positions vector may not be sufficient to recover all the different positions but it may be enough to tell things like the number of positions, their mean and their variance.
\\
\item 
4) A partial sketch of a person, may not have a full sketch of the face, but it may still be enough to get sketch of the eyes if eyes have a high enough weight.
\\
\item 
5) Even if we are not able to recover an object from its sketch, we may get a $O(log n)$ sized sketch or "hash" of it.
So if we have separately stored the sketch of the component object we can use the hash to retrieve the full explicit sketch
\\
\item 
6) Instead of using random R, if we use $(I+R)/2$ then automatically a sketch is close to the sketches of its children and parents.
\end{itemize}

The above properties follow from the following claims:

\begin{claim}\label{claim:sketchproperty1}
Given a sketch of size $\dsketch$, if we erase everything except for prefix of size $\dsketch'$, then any descendent-component of size $s$ and 
``effective weight" $w$ can be recovered completely as long as $f(w,\dsketch') > s$
\end{claim}

Notation: module $M$. Its output is $x_M$ with $\dout$ coordinates, $k_M$ of which are (normalized) one and the rest of which are zero.

\newcommand{\modulestar}{{M^{\star}}}

\josh{Need full knowledge version and quick version.}

\begin{theorem}
  If for some module $\modulestar$, $w_\modulestar^2 \cdot \dsketch \ge k_\modulestar$, then with high probability (over the random matrices), we can efficiently recover $x_\modulestar$ given $s$, all random matrices, and the network hierarchy.
\end{theorem}

\textbf{Basic Proof Idea.}

Recall that our sketch takes the form:
\[
  s = \sum_M f(M) x_M
\]

Since we know $s$, all random matrices, and the network hierarchy, we can compute the inner product of $s$ with $f(\modulestar) e_1$. There's a $\modulestar$ term we care about, and several noise terms.
\[
  \inner{\sum_M f(M) x_M}{f(\modulestar) e_1}
  = e_1^T f(\modulestar)^T f(\modulestar) x_\modulestar
     + \sum_{M \not = \modulestar}
         e_1^T f(\modulestar)^T f(M) x_M
\]
Roughly speaking, $f(\modulestar)$ consists of repeated rotations, so this first term is $w_{\modulestar}^2 e_1^T x_\modulestar$ (in reality, it has some noise as well). Since $x_\modulestar$ is a normalized boolean vector, this gives us a value of $+\frac{w_{\modulestar}^2}{\sqrt{k_{\modulestar}}}$.

Roughly, the other terms are the dot product of two random vectors of norm $w_{\modulestar}$ and $w_M$. Such a dot product is expected to have magnitude $\frac{w_{\modulestar} w_M}{\sqrt{\dsketch}}$. Each dot product has an independently random sign (principle of deferred decisions, with the choice of $R_M$ being the last decision), so the final magnitude of the noise is $\frac{w_{\modulestar} \sqrt{\sum_M w_M}}{\sqrt{\dsketch}} = \frac{w_{\modulestar}}{\sqrt{\dsketch}}$. This is less than the first term is our condition is true, and hence we can value $\left(x_{\modulestar}\right)_1$. We recover the other terms by using $e_2, \ldots, e_{\dsketch}$.

\textbf{Proof Modification Notes.} We could also inner product with $R_M e_1$ if we didn't know the network structure, but then we need the guarantee that each module only appears once! The analysis proceeds in the same manner, essentially only the first term works differently. The condition needs to be stronger by (exponential in depth of module).

\begin{proof}
  Recall that our sketch is:
  \[
    s = \sum_M f(M) x_M
  \]
  
  Since we know $s$, all random matrices, and the network hierarchy, we can compute the inner product of $s$ with
  $f(\modulestar) e_1$.
  \[
    \inner{\sum_M f(M) x_M}{f(\modulestar) e_1}
    = e_1^T f(\modulestar)^T f(\modulestar) x_\modulestar
       + \sum_{M \not = \modulestar}
           e_1^T f(\modulestar)^T f(M) x_M
  \]
  
  Rough Proof: okay, let's unwind each term separately from the center using our Lemmas/Corollaries.
  
  Unwinding the first term. We repeatedly remove the middle pair of matrices. Each time we do, we pick up error proportional to the product of $\ell_2$ norms of the vectors on the two sides. But we know the $\ell_2$ norms are controlled, roughly $(1 \pm \delta)^{3d(M)}$. Hence at worst we pick up $w_\modulestar (1 + \delta)^{6d(M)} \delta$. We chose $\delta$ so that this would be $O(w_\modulestar \delta)$.
  
  Summing over all error terms, we pick up $O(w_\modulestar \delta 3d(\modulestar))$ error.
  
  Remaining terms: The same thing happens. We expect to pick up $O(w_M 3d(M))$ error. Unfortunately, these error terms are not independent; they share matrices. However, their \emph{signs are independent, which is good enough to apply Hoeffding's inequality}. Here's why: even fixing \emph{any magnitudes}, when the signs are random they fulfill the conditions of Hoeffding's inequality anyways.
  
  As a result:
  \[
    \Pr[\text{absolute error} \ge t] \le
      \text{exp}\left(
        2 t^2 / d_\text{max}^2 \delta^2
      \right)
  \]
  
  Hence we get to pick $t = \delta d_\text{max} \log n$.
\end{proof}

\begin{claim}\label{claim:sketchproperty2}
Given a sketch of size $d$, if we erase everything except for prefix of size $d'$, then any descendent-component of size $s$ one can recover
a sketch of that component of size $f(w,d')$. If the full sketch of that component is stored separately in the repository, it will have a high similarity with this sketch and may be retrieved as an indirection.
\end{claim}

\textbf{Basic Proof Idea.} We take the inner product between the two sketches. Our sketches are of the form:
\begin{align*}
  s &= \sum_M f(M) x_M \\
  s' &= \sum_{M'} f(M') x_{M'}
\end{align*}

\josh{First half from main theorem(s), second is just noticing that zeroing stuff out of a vector still leaves decent dot product with itself... also all coordinates are symmetric so zeroing coordinates doesn't target high weight coordinate values.}

\begin{claim}\label{claim:sketchproperty3}
Any descendent-component at depth $h$ has similarity at least $\frac{1}{2^h} w$ with the final sketch. If it is reachable through multiple paths from the root node, this similarity gets added over all those paths.
\end{claim}

\josh{Proof Idea: Break into the $I^h$ terms and the other terms. Expected similarity comes from the former, noise from the latter.}

\begin{claim}\label{claim:sketchproperty4}
If we have a tuple of quantities, then its sketch can be used to obtain simple statistics such as its mean and variance. If we have a set of quantities (such as positions) again its sketch can be used to get an estimate of mean and variance.
\end{claim}

\josh{IIRC, grab the mean from the $I$ part and use that to help deduce the variance... also I don't think this survives normalization?}

\rina{Just assume that it's one layer for mean, same thing for histogramming.}

\begin{claim}\label{claim:sketchproperty5}
If there are $n$ "independent" modules (that are not ancestor, descendants of each other) then the recursive-sketches of their outputs 
have very low correlation: at most $\sqrt{\log n/d}$. For $d = \poly(\log n)$ this is $o(1)$. For a parent, child for appropriate weighting the correlation is much higher. Similarly a sketch of size $d$ and its $d/2$ "erased" sketch is very high: about $1/\sqrt{2}$. Thus if two sketches are similar they refer to some common object to some very similar objects.
\end{claim}

\josh{Proof Idea: Principle of Deferred Decisions on a module matrix.}

Claim 5 shows that sketches are "far apart" unless they represent similar objects. So it is likely that all the object

\begin{theorem}
  If for some $j \in [n]$, $\dsketch \cdot w_j^2 > \sparsity{x_j}$, then given $s$, $R_j$, and $w_j$ we can recover $x_j$ with high probability.
\end{theorem}

\josh{This needs to be made recursive. Leaf nodes of the sketch are binary (aka the outputs of modules), but intermediate nodes can be real valued; we can recover any leaf node with enough weight and given the rotation matrices.}

\begin{proof}
  Consider the inner product
  $X_1 = \inner{\modulesketch{M}}{R_M \ve_1}$.
  \begin{align*}
    X_1 &= \inner{\modulesketch{M}}
                 {R_M \ve_1} \\
        &= \inner{
                   \frac{1}{\sqrt{2}} R_M \transparent{R_1} R_M
                     (1 \oplus y \oplus 00\cdots0)
                   + \frac{1}{\sqrt{2}} R_M \transparent{R_2}
                       \sum_{i=1}^n \frac{1}{\sqrt{n}} \transparent{R_i} \modulesketch{M_j}
                 }
                 {R_M \ve_1}
  \end{align*}
  
  Only one term matters; the expectation of $X_1$ is $\frac{1}{\sqrt{8n}} (\modulesketch{M_j})_1$. Applying Lemma~\ref{lem:apx-rotation} and Lemma~\ref{lem:inner-preserving}, we get that w.h.p. ...
  
  Let's work out the expectation of $X_1$:
  \begin{align*}
    \E{X_1} &= \E{ \frac{w_j(1 + o(1))}{\sqrt{\sparsity{x_j} \log n}} \sum_{k=1}^n \inner{R_j (x_j)_k}{R_j \ve_1} }
             + \underbrace{\E{ \sum_{i \not = j} w_i \inner{\normalize{R_i x_i}}{R_j \ve_1} }}_{=0} \\
            &= \frac{w_j(1 + o(1))}{\sqrt{\sparsity{x_j} \log n}}
               \left[
                 \inner{R_j (x_j)_1}{R_j \ve_1} +
                 \underbrace{\E{ \sum_{k \not = 1}^n \inner{R_j (x_j)_k}{R_j \ve_1} }}_{=0}
               \right] \\
            &= \frac{w_j(1 + o(1))}{\sqrt{\sparsity{x_j} \log n}} (\log n) (x_j)_1 \\
            &= \frac{w_j(\sqrt{\log n})(1 + o(1))}{\sqrt{\sparsity{x_j}}} (x_j)_1
  \end{align*}
  
  As we can see, $X_1$ has an expectation of roughly
  $\frac{w_j \sqrt{\log n}}{\sqrt{\sparsity{x_j}}}$ if $(x_j)_1$ is one and
  zero otherwise.
  
  Nice proof ends here. Rough notes on how to finish:
  \begin{itemize}
      \item Intuitively, we are comparing this 0-1 gap with the noise from the other variables.
      \item Should suffice to use a Chernoff bound...
      \item Think of other coordinates of $x_j$ as another vector $x_i$, since the columns of $R_i$ were chosen independently.
      \item So, we basically have a bunch of $w_i \normalize{R_i x_i}$ to take the inner product with.
      \item This is exactly a weighted sum of independent Bernoulli random variables.
  \end{itemize}
  
  Old proof continuation:

  We can see that this has expectation equal to
  $\frac{w_j}{\sqrt{\sparsity{x_j}}}$ if the first coordinate of $x_j$ is
  one and zero otherwise. Additionally, since the dot product of two uniformly
  random unit vectors has variance $\frac{1}{d}$, this quantity has variance
  $\sum_{i \not = j} \frac{w_i^2}{d} < \frac{1}{d}$.

  Hence, the standard deviation is at most $\frac{1}{\sqrt{d}}$. Comparing this
  to the gap between the coordinate being zero or one, we need:
  \begin{align*}
    \frac{1}{\sqrt{d}} &< \frac{w_j}{\sqrt{\sparsity{x_j}}} \\
    \sparsity{x_j} &< d \cdot w_j^2
  \end{align*}
\end{proof}

==> rina-discussion.tex <==
\section{Discussion}

\psuedosection{Identifying Class/Type Information without explicit type specification from Subspace Components}\label{sec:typeinfo}
The classes supported by our module are not written explicitly but are rather inferred from the subspace corresponding to the object. This gives a ``protocol independent'' way of encoding type/classes into sketches. Moreover, any upstream module can just extract objects of a specific type from the final sketch by projecting the sketch to that specific subspace. This allows us to have ``floating'' modules that are not necessarily hardwired.

\psuedosection{Floating Modules}\label{sec:floatingm}

Modules may be viewed as ``floating'' program functions rather than blocks in a circuit. Unlike the latter floating modules can be  be shared across  different parts of the network. These functions ``listen'' on specific subspaces (like network ports) for objects of certain classes and if there is a match output an object of another class on another subspace (like an output port).
%Can encode a very large network with O(d) size sketches and preserve information from cuts that are sparse, cuts smaller than O(d).
%<Diagram of comparison between communicating modules via neural edges and machines on a broadcast network> Maybe time multiplexing can be used to transfer larger amounts of information over the wires.
Examples of floating modules include:
\begin{enumerate}[nosep]
\item A \emph{counting} module which can approximate the number of copies of an object in an image or the number of times a specific sound occurs. Thus, such a counting block has to be a ``free floating'' module which can feed into any other module in the network.
\item A clustering/dictionary learning module can be used in multiple places to find new concepts or to refine existing ones. 
\item A lines/curves sketcher can be used to sketch curves in images but also the frequency/intensity curve representing a musical segment with respect to time.
\item A SQL-style Projection-GroupBy module: Such a module may be used to take a set of sketches and project out a specific field such as color or texture or velocity and group the sketches by different values according to the resulting projected attributes. It may be used in conjunction with a counting module in order to compress a sketch containing repetitions into a (tuple) sketch corresponding of (count, repeated value) pairs.
\item A modules that listen on a subspace can be thought of as an SQL SELECT operation with a WHERE statement that is looking for specific features. Once such a module is trained, it can feed into essentially any other module in the network.
\end{enumerate}

\psuedosection{Identifying Motion Patterns as Curves in Sketch Space}

Conceptually, a butterfly flapping its wings, a person walking on the street, and a snake slithering on the ground can be identified using this modular view and sketching. Consider a video of a butterfly flapping its wings at a fixed location. Each video frame produces a sketch identifying the butterfly and outputs attributes corresponding it its color, shape, position and the orientation of its wings. Across video frames all that changes is orientation and position of wings. So over time we get a curve in sketch space. Since the video is periodic the curve is actually a loop. Now if we have a module to sketch curves, such a module could take this curve and sketch it into its top few coefficients in say a polynomial or Fourier representation. So the final coefficient sketch would correspond to a flying butterfly. Similar things can happen for any periodic motion such as a person walking (which is periodic once you subtract the velocity vector) or a snake slithering (a periodic motion). Each of these is a specific type of loop in sketch space. In fact this may even be done in an unsupervised fashion: The sketch of a flying butterfly will form a new cluster center in sketch space and can thus be identified as a new module (using previously mentioned ideas).

\psuedosection{Pointers and References}\label{sec:pointers}
A sketch may also serve as a pointer or a reference to a detailed object just like a fingerprint hash. For instance, a short sketch or a large object may be used to uniquely reference a more detailed sketch of that object.
\rina{was there some theorem/claim to move to here?}

\josh{This entire section has been incorporated into the introduction.}

==> tikz-final-sketch.tex <==
% Make it in Google drawings?

==> tikz-module-sketch.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[%
  auto,
  scale=1.0,
  module/.style={
    rectangle,
    draw=blue,
    fill=blue!10,
    inner sep=2pt,
  },
  data/.style={
    ellipse,
    draw=green,
    fill=green!10,
    inner sep=2pt,
  },
  sketch/.style={
    ellipse,
    draw=red,
    fill=red!10,
    inner sep=2pt,
  },
  ]
  %\draw[step=1cm,black!10,very thin] (0, 0) grid (12, 10);

  \node[module] (head-module) at (0, 0) {Module: Head};
  \node[module] (tail-module) at (4, 0) {Module: Tail};
  \node[module] (tiger-module) at (2, 4) {Module: Tiger};

  \node[data] (head-output) at ($(head-module)+(0,2)$) {Head Output};
  \node[data] (tail-output) at ($(tail-module)+(0,2)$) {Tail Output};
  \node[data] (tiger-output) at ($(tiger-module)+(0,2)$) {Tiger Output};
  
  \draw[thick, ->] (head-module) -- (head-output);
  \draw[thick, ->] (tail-module) -- (tail-output);
  
  \draw[thick, ->] (head-output) -- (tiger-module);
  \draw[thick, ->] (tail-output) -- (tiger-module);
  \draw[thick, ->] (tiger-module) -- (tiger-output);

  \node[sketch] (head-sketch) at (8, 0) {Sketch: Head};
  \node[sketch] (tail-sketch) at (12, 0) {Sketch: Tail};
  \node[sketch] (children) at (10, 2) {};
  \node[sketch] (rotated) at ($(tiger-output)+(4, 0)$) {};
  \node[sketch] (almost) at (8, 4) {};
  \node[sketch] (tiger-sketch) at (10, 6) {Sketch: Tiger};
  
  \draw[thick, ->]
    (head-sketch) --
    node[above left] {$\onetwo \transparent{R_1}$}
    (children);
  \draw[thick, ->]
    (tail-sketch) --
    node[above right] {$\onetwo \transparent{R_2}$}
    (children);
  \draw[thick, ->]
    (tiger-output) --
    node[above] {$R_{\text{tiger}}$}
    (rotated);
  \draw[thick, ->]
    (rotated) --
    node[below left] {$\onetwo \transparent{R_1}$}
    (almost);
  \draw[thick, ->]
    (children) --
    node[below left] {$\onetwo \transparent{R_2}$}
    (almost);
  \draw[thick, ->]
    (almost) --
    node[below right] {$\transparent{R_\text{tiger}}$}
    (tiger-sketch);
\end{tikzpicture}
\caption{Recursive sketch example. This tiger module sits on top of the head and tail modules. Its recursive sketch is based on its output and the recursive sketches of its children.}
\label{fig:module-sketch}
\end{figure}

==> tikz-tuple-sketch.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[%
  auto,
  scale=1.0,
  sketch/.style={
    ellipse,
    draw=red,
    fill=red!10,
    inner sep=2pt,
  },
  ]
  %\draw[step=1cm,black!10,very thin] (0, 0) grid (12, 10);

  \node[sketch] (sketch1) at (0, 0) {Sketch $1$};
  \node[sketch] (sketch2) at (4, 0) {Sketch $2$};
  \node (sketch3) at (8, 0) {$\cdots$};
  \node[sketch] (sketch4) at (12, 0) {Sketch $n$};
  
  \node[sketch] (tuple-sketch) at (6, 2) {Tuple Sketch};
  
  \draw[thick, ->]
    (sketch1) --
    node[above left]
      {$\frac{1}{\sqrt{n}} \transparent{R_1}$}
    (tuple-sketch);
  \draw[thick, ->]
    (sketch2) --
    node[below right]
      {$\frac{1}{\sqrt{n}} \transparent{R_2}$}
    (tuple-sketch);
  \draw[thick, ->]
    (sketch4) --
    node[above right]
      {$\frac{1}{\sqrt{n}} \transparent{R_n}$}
    (tuple-sketch);
\end{tikzpicture}
\caption{Balanced tuple sketch.}
\label{fig:tuple-sketch}
\end{figure}
